Smooth Combs Inside Hedgehogs

We use techniques of tube-log Riemann surfaces due to R.Perez-Marco to construct a hedgehog containing smooth $C^{\infty}$ combs. The hedgehog is a common hedgehog for a family of commuting non-linearisable holomorphic maps with a common indifferent fixed point. The comb is made up of smooth curves, and is transversally bi-H\"older regular.

==> defv7.tex <==
\def\D{\Delta} 
\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
\def\l{\ell}
\def\G{\Gamma}
\def\g{\gamma}
\def\eps{\varepsilon}
\def\t{\theta}
\def\O{\Omega}
\def\o{\omega}
\def\w{\omega}
\def\ll{\lambda}
\def\L{\Lambda}
\def\s{\sigma}
\def\S{\Sigma}


\def \dd#1{{\bf#1}}

\def\cl#1{{\cal#1}} 


%Simbolos matematicos.

\def\ge{f(z)=\ll z +\cO(z^2)}
\def\geg{g(z)=\mu z +\cO(z^2)}
\def\tilda{\tilde}
\def\ti{\tilde}
\def\ea{e^{2\pi i \alpha}}
\def\eb{e^{2\pi i \beta}}
\def\der{\partial}
\def\LRA{\Leftrightarrow}
\def\gea{f(z)=\ea z +\c O (z^2)}




\def\cdm{{1\over 2\pi}\sum_{i=0}^n \b_{i-1}\llog
		     (e\a_i^{-1})-C}
\def\cdi{\sum_{n=1}^{+\infty}{\llog q_{n+1}\over 
	q_n}}

\def\adh{\mathop{\rm adh}\nolimits}
\def\llog{\mathop{\rm loglog}\nolimits}
\def\mod{\mathop{\rm mod}\nolimits}
\def\Max{\mathop{\rm Max}}
\def\Min{\mathop{\rm Min}}
\def\Sup{\mathop{\rm Sup}}
\def\Tor{\mathop{\rm Tor}}
\def\Inf{\mathop{\rm Inf}}
\def\diam{\mathop{\rm diam}}
\def\rang{\mathop{\rm rang}}
\def\Pic{\mathop{\rm Pic}}
\def\Det{\mathop{\rm Det}}
\def\det{\mathop{\rm det}}
\def\Aut{\mathop{\rm Aut}}
\def\Arg{\mathop{\rm Arg}\nolimits}
\def\Cent{\mathop{\rm Cent}\nolimits}
\def\Centf{\mathop{\rm Cent}_{\rm f}\nolimits}
\def\Diff{\mathop{\rm Diff}\nolimits}

\def\Im{\mathop{\rm Im}\nolimits}
\def\Re{\mathop{\rm Re}\nolimits}
\def\id{\mathop{\rm id}\nolimits}


%Macros.

\def\ouv#1{\smash{\mathop{#1}\limits^{\lower 1pt\hbox
{$\scriptscriptstyle\circ$}}}}

\def\apl#1#2#3#4#5{{#1}:\matrix{
		\hfill#2 & \longrightarrow & #3\hfill \cr
		\hfill#4 & \longmapsto     & #5\hfill \cr}}


\def\ap#1#2#3#4{\matrix{
		\hfill#1 & \longrightarrow & #2\hfill \cr
		\hfill#3 & \longmapsto     & #4\hfill \cr}}


\def\uple#1#2{({#1}_1,{#1}_2,\ldots ,{#1}_{#2})}

\def\fuple#1#2#3{{#1}_{{#2}_1}\circ {#1}_{{#2}_2}\circ \ldots 
\circ {#1}_{{#2}_{#3}}}

\def\ffuple#1#2#3#4{{#1}_{{#2},{#3}_1}\circ 
{#1}_{{#2},{#3}_2}\circ \ldots \circ {#1}_{{#2},{#3}_{#4}}}



\def\hfl#1#2{\smash{\mathop{\hbox to 12mm{\rightarrowfill}}
\limits^{\scriptstyle#1}_{\scriptstyle#2}}}

\def\vfl#1#2{\llap{$\scriptstyle#1$}\left\downarrow
\vbox to 6mm{}\right.\rlap{$\scriptstyle #2$}}

\def\diagram#1{\def\normalbaselines{\baselineskip=0pt
\lineskip=10pt\lineskiplimit=1pt}  \matrix{#1}}





%Titulos, enunciados.


\long\def\eno#1#2{\par\smallskip{\bf{#1}}{\it\ {#2}}\par\medskip}

\def\tit#1{\vskip 5mm plus 1mm minus 2mm {\tir #1}
		\vskip 3mm plus 1mm minus 2mm}

\def\stit#1{\vskip 3mm plus 1mm minus 2mm {\bf{#1}}
		\smallskip}

\def\Stit#1{\vskip 2cm
\centerline{\tir {#1}}\vskip 2cm 
plus 5mm minus 2mm}



\def\Stitl#1#2{\vskip 2cm
\centerline{\tir {#1}}

\centerline{\tir {#2}}\vskip 2cm 
plus 5mm minus 2mm}


\def\Stitm#1{\vskip 1cm
\centerline{\tir {#1}}\vskip 1cm 
plus 2mm minus 2mm}

\long\def\dem#1#2{{\bf {#1}}{\ {#2}$\diamondsuit$}\medskip}

\font\tir=cmbx10 at 12pt

\font\tirr=cmbx10 at 18pt


\long\def\ctitre#1{\vbox{\leftskip=0pt plus 1fil
\rightskip=0ptplus 1fil \parfillskip=0pt#1}}

\def\ref#1#2#3#4{{\bf #1}{\ #2}{\it ,\ #3}{,\ #4}\medskip}


%Dibujos

\def \picture #1 by #2 (#3){\midinsert \centerline 
{\vbox to #2{\hrule width #1 heigth 0pt 
depth 0pt \null \vfill \special {picture #3}}}\endinsert }

\def\scaledpicture #1 by #2 (#3 scaled #4) {{
\dimen0 =#1 \dimen1 =$2
\divide \dimen0 by 1000 \multiply \dimen0 by #4
\divide \dimen1 by 1000 \multiply \dimen1 by #4
\picture \dimen0 by \dimen1 (#3 scaled $4)}}

%\def\figure #1 #2{\scaledpicture 80cm by 8cm (#1 scaled #2)}

\def\figure #1 #2 #3 {\midinsert \vglue 3mm 
{\vbox to #3 {\hrule width 6cm height 0cm depth 0cm \vfill
{\special {picture #1 scaled #2}}}}\vglue 2mm \endinsert}

\magnification=1200






